Joint Determination of Reactor Antineutrino Spectra from $^{235}$U and $^{239}$Pu Fission by Daya Bay and PROSPECT

A joint determination of the reactor antineutrino spectra resulting from the fission of $^{235}$U and $^{239}$Pu has been carried out by the Daya Bay and PROSPECT collaborations. This Letter reports the level of consistency of $^{235}$U spectrum measurements from the two experiments and presents new results from a joint analysis of both data sets. The measurements are found to be consistent. The combined analysis reduces the degeneracy between the dominant $^{235}$U and $^{239}$Pu isotopes and improves the uncertainty of the $^{235}$U spectral shape to about 3\%. The ${}^{235}$U and $^{239}$Pu antineutrino energy spectra are unfolded from the jointly deconvolved reactor spectra using the Wiener-SVD unfolding method, providing a data-based reference for other reactor antineutrino experiments and other applications. This is the first measurement of the $^{235}$U and $^{239}$Pu spectra based on the combination of experiments at low- and highly enriched uranium reactors.

==> Daya Bay - PROSPECT Joint Spectrum Measurement/merged_prospect_dyb_authors.tex <==
%%%% Generator info for file
%%%% Thu Apr  8 09:27:29 2021
%%%% /Users/djaffe/Documents/Reactor/work/trunk/NuWa-trunk/dybgaudi/Documentation/AuthorList_SAVE/2021_PROSPECT_DYB_Spectrum
%%%% merge.py 
%
\newcommand{\NUU}{\affiliation{National~United~University, Miao-Li}}
\newcommand{\NIST}{\affiliation{National Institute of Standards and Technology, Gaithersburg, MD, USA}}
\newcommand{\UCB}{\affiliation{Department of Physics, University~of~California, Berkeley, California  94720, USA}}
\newcommand{\Hawaii}{\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, HI, USA}}
\newcommand{\IIT}{\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, IL, USA}}
\newcommand{\SJTU}{\affiliation{Department of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai Laboratory for Particle Physics and Cosmology, Shanghai}}
\newcommand{\HKU}{\affiliation{Department of Physics, The~University~of~Hong~Kong, Pokfulam, Hong~Kong}}
\newcommand{\UCI}{\affiliation{Department of Physics and Astronomy, University of California, Irvine, California 92697, USA}} %20190209 for Pedro's new digs
\newcommand{\TsingHua}{\affiliation{Department~of~Engineering~Physics, Tsinghua~University, Beijing}}
\newcommand{\VirginiaTech}{\affiliation{Center for Neutrino Physics, Virginia~Tech, Blacksburg, Virginia  24061, USA}}
\newcommand{\ORNL}{\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
\newcommand{\NJU}{\affiliation{Nanjing~University, Nanjing}}
\newcommand{\ECUST}{\affiliation{Institute of Modern Physics, East China University of Science and Technology, Shanghai}}
\newcommand{\CUHK}{\affiliation{Chinese~University~of~Hong~Kong, Hong~Kong}}
\newcommand{\UIUC}{\affiliation{Department of Physics, University~of~Illinois~at~Urbana-Champaign, Urbana, Illinois 61801, USA}}
\newcommand{\Drexel}{\affiliation{Department of Physics, Drexel University, Philadelphia, PA, USA}}
\newcommand{\HFIR}{\affiliation{High Flux Isotope Reactor, Oak Ridge National Laboratory, Oak Ridge, TN, USA}}
\newcommand{\BNL}{\affiliation{Brookhaven National Laboratory, Upton, NY, USA}}
\newcommand{\NUDT}{\affiliation{College of Electronic Science and Engineering, National University of Defense Technology, Changsha}} % added 20140111
\newcommand{\CIAE}{\affiliation{China~Institute~of~Atomic~Energy, Beijing}}
\newcommand{\TENN}{\affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, TN, USA}}
\newcommand{\GXU}{\affiliation{Guangxi University, No.100 Daxue East Road, Nanning}} % added 20201208 ,530004, China
\newcommand{\BNU}{\affiliation{Beijing~Normal~University, Beijing}}
\newcommand{\Iowa}{\affiliation{Iowa~State~University, Ames, Iowa  50011, USA}}
\newcommand{\ZSU}{\affiliation{Sun Yat-Sen (Zhongshan) University, Guangzhou}}
\newcommand{\NanKai}{\affiliation{School of Physics, Nankai~University, Tianjin}}
\newcommand{\TempleUniversity}{\affiliation{Department of Physics, Temple University, Philadelphia, PA, USA}}
\newcommand{\GATECH}{\affiliation{George W.\,Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, GA USA}}
\newcommand{\DGUT}{\affiliation{Dongguan~University~of~Technology, Dongguan}}
\newcommand{\UC}{\affiliation{Department of Physics, University~of~Cincinnati, Cincinnati, Ohio 45221, USA}}
\newcommand{\BCC}{\altaffiliation{Now at Department of Chemistry and Chemical Technology, Bronx Community College, Bronx, New York  10453, USA}} % add 20160311 for Sunej's 'now at'
\newcommand{\NCTU}{\affiliation{Institute~of~Physics, National~Chiao-Tung~University, Hsinchu}}
\newcommand{\XJTU}{\affiliation{Department of Nuclear Science and Technology, School of Energy and Power Engineering, Xi'an Jiaotong University, Xi'an}}%%updated 20161215 {Xi'an Jiaotong University, Xi'an}}
\newcommand{\LLNL}{\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, CA, USA}}
\newcommand{\Waterloo}{\affiliation{Institute for Quantum Computing and Department of Physics and Astronomy, University of Waterloo, Waterloo, ON, Canada}}
\newcommand{\Berkeley}{\affiliation{Lawrence~Berkeley~National~Laboratory, Berkeley, California 94720, USA}}
\newcommand{\Charles}{\affiliation{Charles~University, Faculty~of~Mathematics~and~Physics, Prague, Czech Republic}} %updated20140819
\newcommand{\CGNPG}{\affiliation{China General Nuclear Power Group, Shenzhen}}% update 20170729 add city. updated 20140724 China~Guangdong~Nuclear~Power~Group, Shenzhen}}
\newcommand{\Yale}{\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, CT, USA}}
\newcommand{\Wisconsin}{\affiliation{Department of Physics, University of Wisconsin, Madison, Madison, WI, USA}}
\newcommand{\Dubna}{\affiliation{Joint~Institute~for~Nuclear~Research, Dubna, Moscow~Region, Russia}}
\newcommand{\LeMoyne}{\affiliation{Department of Physics, Le Moyne College, Syracuse, NY, USA}}
\newcommand{\NTU}{\affiliation{Department of Physics, National~Taiwan~University, Taipei}}
\newcommand{\Princeton}{\affiliation{Joseph Henry Laboratories, Princeton~University, Princeton, New~Jersey 08544, USA}}
\newcommand{\SDU}{\affiliation{Shandong~University, Jinan}}
\newcommand{\CNIHEP}{\affiliation{Institute~of~High~Energy~Physics, Beijing}}
\newcommand{\CQU}{\affiliation{Chongqing University, Chongqing}} % add 20150417
\newcommand{\Siena}{\affiliation{Siena~College, Loudonville, New York  12211, USA}}
\newcommand{\NCEPU}{\affiliation{North~China~Electric~Power~University, Beijing}}
\newcommand{\Caltech}{\affiliation{California~Institute~of~Technology, Pasadena, California 91125, USA}}
\newcommand{\WandM}{\affiliation{College~of~William~and~Mary, Williamsburg, Virginia  23187, USA}}
\newcommand{\SZU}{\affiliation{Shenzhen~University, Shenzhen}}
\newcommand{\USTC}{\affiliation{University~of~Science~and~Technology~of~China, Hefei}}
%
\author{F.~P.~An\ensuremath{^{\delta}}}
\ECUST 
\author{M.~Andriamirado\ensuremath{^{\pi}}}
\IIT 
\author{A.~B.~Balantekin\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\Wisconsin 
\author{H.~R.~Band\ensuremath{^{\pi}}}
\Yale 
\author{C.~D.~Bass\ensuremath{^{\pi}}}
\LeMoyne 
\author{D.~E.~Bergeron\ensuremath{^{\pi}}}
\NIST 
\author{D.~Berish\ensuremath{^{\pi}}}
\TempleUniversity 
\author{M.~Bishai\ensuremath{^{\delta}}}
\BNL 
\author{S.~Blyth\ensuremath{^{\delta}}}
\NTU 
\author{N.~S.~Bowden\ensuremath{^{\pi}}}
\LLNL 
\author{C.~D.~Bryan\ensuremath{^{\pi}}}
\HFIR 
\author{G.~F.~Cao\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~Cao\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~F.~Chang\ensuremath{^{\delta}}}
\CNIHEP 
\author{Y.~Chang\ensuremath{^{\delta}}}
\NUU 
\author{H.~S.~Chen\ensuremath{^{\delta}}}
\CNIHEP 
\author{S.~M.~Chen\ensuremath{^{\delta}}}
\TsingHua 
\author{Y.~Chen\ensuremath{^{\delta}}}
\SZU\ZSU 
\author{Y.~X.~Chen\ensuremath{^{\delta}}}
\NCEPU 
\author{J.~Cheng\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~K.~Cheng\ensuremath{^{\delta}}}
\ZSU 
\author{J.~J.~Cherwinka\ensuremath{^{\delta}}}
\Wisconsin 
\author{M.~C.~Chu\ensuremath{^{\delta}}}
\CUHK 
\author{T.~Classen\ensuremath{^{\pi}}}
\LLNL 
\author{A.~J.~Conant\ensuremath{^{\pi}}}
\HFIR 
\author{J.~P.~Cummings\ensuremath{^{\delta}}}
\Siena 
\author{O.~Dalager\ensuremath{^{\delta}}}
\UCI 
\author{G.~Deichert\ensuremath{^{\pi}}}
\HFIR 
\author{A.~Delgado\ensuremath{^{\pi}}}
\ORNL\TENN
\author{F.~S.~Deng\ensuremath{^{\delta}}}
\USTC 
\author{Y.~Y.~Ding\ensuremath{^{\delta}}}
\CNIHEP 
\author{M.~V.~Diwan\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{T.~Dohnal\ensuremath{^{\delta}}}
\Charles 
\author{M.~J.~Dolinski\ensuremath{^{\pi}}}
\Drexel 
\author{D.~Dolzhikov\ensuremath{^{\delta}}}
\Dubna 
\author{J.~Dove\ensuremath{^{\delta}}}
\UIUC 
\author{M.~Dvo\v{r}\'{a}k\ensuremath{^{\delta}}}
\CNIHEP 
\author{D.~A.~Dwyer\ensuremath{^{\delta}}}
\Berkeley 
\author{A.~Erickson\ensuremath{^{\pi}}}
\GATECH 
\author{B.~T.~Foust\ensuremath{^{\pi}}}
\Yale 
\author{J.~K.~Gaison\ensuremath{^{\pi}}}
\Yale 
\author{A.~Galindo-Uribarri\ensuremath{^{\pi}}}
\ORNL\TENN 
\author{J.~P.~Gallo\ensuremath{^{\delta}}}
\IIT 
\author{C.~E.~Gilbert\ensuremath{^{\pi}}}
\ORNL\TENN 
\author{M.~Gonchar\ensuremath{^{\delta}}}
\Dubna 
\author{G.~H.~Gong\ensuremath{^{\delta}}}
\TsingHua 
\author{H.~Gong\ensuremath{^{\delta}}}
\TsingHua 
\author{M.~Grassi\ensuremath{^{\delta}}}
\UCI 
\author{W.~Q.~Gu\ensuremath{^{\delta}}}
\BNL 
\author{J.~Y.~Guo\ensuremath{^{\delta}}}
\ZSU 
\author{L.~Guo\ensuremath{^{\delta}}}
\TsingHua 
\author{X.~H.~Guo\ensuremath{^{\delta}}}
\BNU 
\author{Y.~H.~Guo\ensuremath{^{\delta}}}
\XJTU 
\author{Z.~Guo\ensuremath{^{\delta}}}
\TsingHua 
\author{R.~W.~Hackenburg\ensuremath{^{\delta}}}
\BNL 
\author{S.~Hans\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BCC\BNL 
\author{A.~B.~Hansell\ensuremath{^{\pi}}}
\TempleUniversity 
\author{M.~He\ensuremath{^{\delta}}}
\CNIHEP 
\author{K.~M.~Heeger\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\Yale 
\author{B.~Heffron\ensuremath{^{\pi}}}
\ORNL\TENN 
\author{Y.~K.~Heng\ensuremath{^{\delta}}}
\CNIHEP 
\author{Y.~K.~Hor\ensuremath{^{\delta}}}
\ZSU 
\author{Y.~B.~Hsiung\ensuremath{^{\delta}}}
\NTU 
\author{B.~Z.~Hu\ensuremath{^{\delta}}}
\NTU 
\author{J.~R.~Hu\ensuremath{^{\delta}}}
\CNIHEP 
\author{T.~Hu\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~J.~Hu\ensuremath{^{\delta}}}
\ZSU 
\author{H.~X.~Huang\ensuremath{^{\delta}}}
\CIAE 
\author{J.~H.~Huang\ensuremath{^{\delta}}}
\CNIHEP 
\author{X.~T.~Huang\ensuremath{^{\delta}}}
\SDU 
\author{Y.~B.~Huang\ensuremath{^{\delta}}}
\GXU 
\author{P.~Huber\ensuremath{^{\delta}}}
\VirginiaTech 
\author{J. Koblanski\ensuremath{^{\pi}}}
\Hawaii 
\author{D.~E.~Jaffe\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{S.~Jayakumar\ensuremath{^{\pi}}}
\Drexel 
\author{K.~L.~Jen\ensuremath{^{\delta}}}
\NCTU 
\author{X.~L.~Ji\ensuremath{^{\delta}}}
\CNIHEP 
\author{X.~P.~Ji\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{R.~A.~Johnson\ensuremath{^{\delta}}}
\UC 
\author{D.~C.~Jones\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\TempleUniversity 
\author{L.~Kang\ensuremath{^{\delta}}}
\DGUT 
\author{S.~H.~Kettell\ensuremath{^{\delta}}}
\BNL 
\author{S.~Kohn\ensuremath{^{\delta}}}
\UCB 
\author{M.~Kramer\ensuremath{^{\delta}}}
\Berkeley\UCB 
\author{O.~Kyzylova\ensuremath{^{\pi}}}
\Drexel 
\author{C.~E.~Lane\ensuremath{^{\pi}}}
\Drexel 
\author{T.~J.~Langford\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\Yale 
\author{J.~LaRosa\ensuremath{^{\pi}}}
\NIST 
\author{J.~Lee\ensuremath{^{\delta}}}
\Berkeley 
\author{J.~H.~C.~Lee\ensuremath{^{\delta}}}
\HKU 
\author{R.~T.~Lei\ensuremath{^{\delta}}}
\DGUT 
\author{R.~Leitner\ensuremath{^{\delta}}}
\Charles 
\author{J.~K.~C.~Leung\ensuremath{^{\delta}}}
\HKU 
\author{F.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{H.~L.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~J.~Li\ensuremath{^{\delta}}}
\TsingHua 
\author{Q.~J.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{R.~H.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{S.~Li\ensuremath{^{\delta}}}
\DGUT 
\author{S.~C.~Li\ensuremath{^{\delta}}}
\VirginiaTech 
\author{W.~D.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{X.~N.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{X.~Q.~Li\ensuremath{^{\delta}}}
\NanKai 
\author{Y.~F.~Li\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~B.~Li\ensuremath{^{\delta}}}
\ZSU 
\author{H.~Liang\ensuremath{^{\delta}}}
\USTC 
\author{C.~J.~Lin\ensuremath{^{\delta}}}
\Berkeley 
\author{G.~L.~Lin\ensuremath{^{\delta}}}
\NCTU 
\author{S.~Lin\ensuremath{^{\delta}}}
\DGUT 
\author{J.~J.~Ling\ensuremath{^{\delta}}}
\ZSU 
\author{J.~M.~Link\ensuremath{^{\delta}}}
\VirginiaTech 
\author{L.~Littenberg\ensuremath{^{\delta}}}
\BNL 
\author{B.~R.~Littlejohn\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\IIT 
\author{J.~C.~Liu\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~L.~Liu\ensuremath{^{\delta}}}
\SJTU 
\author{J.~X.~Liu\ensuremath{^{\delta}}}
\CNIHEP 
\author{C.~Lu\ensuremath{^{\delta}}}
\Princeton 
\author{H.~Q.~Lu\ensuremath{^{\delta}}}
\CNIHEP 
\author{X.~Lu\ensuremath{^{\pi}}}
\ORNL\TENN 
\author{K.~B.~Luk\ensuremath{^{\delta}}}
\UCB\Berkeley 
\author{B.~Z.~Ma\ensuremath{^{\delta}}}
\SDU 
\author{X.~B.~Ma\ensuremath{^{\delta}}}
\NCEPU 
\author{X.~Y.~Ma\ensuremath{^{\delta}}}
\CNIHEP 
\author{Y.~Q.~Ma\ensuremath{^{\delta}}}
\CNIHEP 
\author{R.~C.~Mandujano\ensuremath{^{\delta}}}
\UCI 
\author{J.~Maricic\ensuremath{^{\pi}}}
\Hawaii 
\author{C.~Marshall\ensuremath{^{\delta}}}
\Berkeley 
\author{K.~T.~McDonald\ensuremath{^{\delta}}}
\Princeton 
\author{R.~D.~McKeown\ensuremath{^{\delta}}}
\Caltech\WandM 
\author{M.~P.~Mendenhall\ensuremath{^{\pi}}}
\LLNL 
\author{Y.~Meng\ensuremath{^{\delta}}}
\SJTU 
\author{A.~M.~Meyer\ensuremath{^{\pi}}}
\Hawaii 
\author{R.~Milincic\ensuremath{^{\pi}}}
\Hawaii 
\author{P.~E.~Mueller\ensuremath{^{\pi}}}
\ORNL 
\author{H.~P.~Mumm\ensuremath{^{\pi}}}
\NIST 
\author{J.~Napolitano\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\TempleUniversity 
\author{D.~Naumov\ensuremath{^{\delta}}}
\Dubna 
\author{E.~Naumova\ensuremath{^{\delta}}}
\Dubna 
\author{R.~Neilson\ensuremath{^{\pi}}}
\Drexel 
\author{T.~M.~T.~Nguyen\ensuremath{^{\delta}}}
\NCTU 
\author{J.~A.~Nikkel\ensuremath{^{\pi}}}
\Yale 
\author{S.~Nour\ensuremath{^{\pi}}}
\NIST 
\author{J.~P.~Ochoa-Ricoux\ensuremath{^{\delta}}}
\UCI 
\author{A.~Olshevskiy\ensuremath{^{\delta}}}
\Dubna 
\author{J.~L.~Palomino\ensuremath{^{\pi}}}
\IIT 
\author{H.-R.~Pan\ensuremath{^{\delta}}}
\NTU 
\author{J.~Park\ensuremath{^{\delta}}}
\VirginiaTech 
\author{S.~Patton\ensuremath{^{\delta}}}
\Berkeley 
\author{J.~C.~Peng\ensuremath{^{\delta}}}
\UIUC 
\author{C.~S.~J.~Pun\ensuremath{^{\delta}}}
\HKU 
\author{D.~A.~Pushin\ensuremath{^{\pi}}}
\Waterloo 
\author{F.~Z.~Qi\ensuremath{^{\delta}}}
\CNIHEP 
\author{M.~Qi\ensuremath{^{\delta}}}
\NJU 
\author{X.~Qian\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{N.~Raper\ensuremath{^{\delta}}}
\ZSU 
\author{J.~Ren\ensuremath{^{\delta}}}
\CIAE 
\author{C.~Morales~Reveco\ensuremath{^{\delta}}}
\UCI 
\author{R.~Rosero\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{B.~Roskovec\ensuremath{^{\delta}}}
\UCI 
\author{X.~C.~Ruan\ensuremath{^{\delta}}}
\CIAE 
\author{M.~Searles\ensuremath{^{\pi}}}
\HFIR
\author{H.~Steiner\ensuremath{^{\delta}}}
\UCB\Berkeley 
\author{J.~L.~Sun\ensuremath{^{\delta}}}
\CGNPG 
\author{P.~T.~Surukuchi\ensuremath{^{\pi}}}
\Yale 
\author{T.~Tmej\ensuremath{^{\delta}}}
\Charles 
\author{K.~Treskov\ensuremath{^{\delta}}}
\Dubna 
\author{W.-H.~Tse\ensuremath{^{\delta}}}
\CUHK 
\author{C.~E.~Tull\ensuremath{^{\delta}}}
\Berkeley 
\author{M.~A.~Tyra\ensuremath{^{\pi}}}
\NIST 
\author{R.~L.~Varner\ensuremath{^{\pi}}}
\ORNL 
\author{D.~Venegas-Vargas\ensuremath{^{\pi}}}
\ORNL\TENN 
\author{B.~Viren\ensuremath{^{\delta}}}
\BNL 
\author{V.~Vorobel\ensuremath{^{\delta}}}
\Charles 
\author{C.~H.~Wang\ensuremath{^{\delta}}}
\NUU 
\author{J.~Wang\ensuremath{^{\delta}}}
\ZSU 
\author{M.~Wang\ensuremath{^{\delta}}}
\SDU 
\author{N.~Y.~Wang\ensuremath{^{\delta}}}
\BNU 
\author{R.~G.~Wang\ensuremath{^{\delta}}}
\CNIHEP 
\author{W.~Wang\ensuremath{^{\delta}}}
\ZSU\WandM 
\author{W.~Wang\ensuremath{^{\delta}}}
\NJU 
\author{X.~Wang\ensuremath{^{\delta}}}
\NUDT 
\author{Y.~Wang\ensuremath{^{\delta}}}
\NJU 
\author{Y.~F.~Wang\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~Wang\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~Wang\ensuremath{^{\delta}}}
\TsingHua 
\author{Z.~M.~Wang\ensuremath{^{\delta}}}
\CNIHEP 
\author{P.~B.~Weatherly\ensuremath{^{\pi}}}
\Drexel 
\author{H.~Y.~Wei\ensuremath{^{\delta}}}
\BNL 
\author{L.~H.~Wei\ensuremath{^{\delta}}}
\CNIHEP 
\author{L.~J.~Wen\ensuremath{^{\delta}}}
\CNIHEP 
\author{K.~Whisnant\ensuremath{^{\delta}}}
\Iowa 
\author{C.~White\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\IIT 
\author{J.~Wilhelmi\ensuremath{^{\pi}}}
\Yale 
\author{H.~L.~H.~Wong\ensuremath{^{\delta}}}
\UCB\Berkeley 
\author{A.~Woolverton\ensuremath{^{\pi}}}
\Waterloo 
\author{E.~Worcester\ensuremath{^{\delta}}}
\BNL 
\author{D.~R.~Wu\ensuremath{^{\delta}}}
\CNIHEP 
\author{F.~L.~Wu\ensuremath{^{\delta}}}
\NJU 
\author{Q.~Wu\ensuremath{^{\delta}}}
\SDU 
\author{W.~J.~Wu\ensuremath{^{\delta}}}
\CNIHEP 
\author{D.~M.~Xia\ensuremath{^{\delta}}}
\CQU 
\author{Z.~Q.~Xie\ensuremath{^{\delta}}}
\CNIHEP 
\author{Z.~Z.~Xing\ensuremath{^{\delta}}}
\CNIHEP 
\author{H.~K.~Xu\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~L.~Xu\ensuremath{^{\delta}}}
\CNIHEP 
\author{T.~Xu\ensuremath{^{\delta}}}
\TsingHua 
\author{T.~Xue\ensuremath{^{\delta}}}
\TsingHua 
\author{C.~G.~Yang\ensuremath{^{\delta}}}
\CNIHEP 
\author{L.~Yang\ensuremath{^{\delta}}}
\DGUT 
\author{Y.~Z.~Yang\ensuremath{^{\delta}}}
\TsingHua 
\author{H.~F.~Yao\ensuremath{^{\delta}}}
\CNIHEP 
\author{M.~Ye\ensuremath{^{\delta}}}
\CNIHEP 
\author{M.~Yeh\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{B.~L.~Young\ensuremath{^{\delta}}}
\Iowa 
\author{H.~Z.~Yu\ensuremath{^{\delta}}}
\ZSU 
\author{Z.~Y.~Yu\ensuremath{^{\delta}}}
\CNIHEP 
\author{B.~B.~Yue\ensuremath{^{\delta}}}
\ZSU 
\author{V.~Zavadskyi\ensuremath{^{\delta}}}
\Dubna 
\author{S.~Zeng\ensuremath{^{\delta}}}
\CNIHEP 
\author{Y.~Zeng\ensuremath{^{\delta}}}
\ZSU 
\author{L.~Zhan\ensuremath{^{\delta}}}
\CNIHEP 
\author{C.~Zhang\ensuremath{^{\delta}}\ensuremath{^{\pi}}}
\BNL 
\author{F.~Y.~Zhang\ensuremath{^{\delta}}}
\SJTU 
\author{H.~H.~Zhang\ensuremath{^{\delta}}}
\ZSU 
\author{J.~W.~Zhang\ensuremath{^{\delta}}}
\CNIHEP 
\author{Q.~M.~Zhang\ensuremath{^{\delta}}}
\XJTU 
\author{S.~Q.~Zhang\ensuremath{^{\delta}}}
\ZSU 
\author{X.~Zhang\ensuremath{^{\pi}}}
\LLNL 
\author{X.~T.~Zhang\ensuremath{^{\delta}}}
\CNIHEP 
\author{Y.~M.~Zhang\ensuremath{^{\delta}}}
\ZSU 
\author{Y.~X.~Zhang\ensuremath{^{\delta}}}
\CGNPG 
\author{Y.~Y.~Zhang\ensuremath{^{\delta}}}
\SJTU 
\author{Z.~J.~Zhang\ensuremath{^{\delta}}}
\DGUT 
\author{Z.~P.~Zhang\ensuremath{^{\delta}}}
\USTC 
\author{Z.~Y.~Zhang\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~Zhao\ensuremath{^{\delta}}}
\CNIHEP 
\author{R.~Z.~Zhao\ensuremath{^{\delta}}}
\CNIHEP 
\author{L.~Zhou\ensuremath{^{\delta}}}
\CNIHEP 
\author{H.~L.~Zhuang\ensuremath{^{\delta}}}
\CNIHEP 
\author{J.~H.~Zou\ensuremath{^{\delta}}}
\CNIHEP 
%
\collaboration{\ensuremath{^{\delta}}Daya Bay Collaboration}\noaffiliation
\collaboration{\ensuremath{^{\pi}}PROSPECT Collaboration}\noaffiliation

